ThinkRepair: Self-Directed Automated Program Repair

Though many approaches have been proposed for Automated Program Repair (APR) and indeed achieved remarkable performance, they still have limitations in fixing bugs that require analyzing and reasoning about the logic of the buggy program. Recently, large language models (LLMs) instructed by prompt engineering have attracted much attention for their powerful ability to address many kinds of tasks including bug-fixing. However, the quality of the prompt will highly affect the ability of LLMs and manually constructing high-quality prompts is a costly endeavor. To address this limitation, we propose a self-directed LLM-based automated program repair, ThinkRepair, with two main phases: collection phase and fixing phase. The former phase automatically collects various chains of thoughts that constitute pre-fixed knowledge by instructing LLMs with the Chain-of-Thought (CoT) prompt. The latter phase targets fixing a bug by first selecting examples for few-shot learning and second automatically interacting with LLMs, optionally appending with feedback of testing information. Evaluations on two widely studied datasets (Defects4J and QuixBugs) by comparing ThinkRepair with 12 SOTA APRs indicate the priority of ThinkRepair in fixing bugs. Notably, ThinkRepair fixes 98 bugs and improves baselines by 27%-344.4% on Defects4J V1.2. On Defects4J V2.0, ThinkRepair fixes 12-65 more bugs than the SOTA APRs. Additionally, ThinkRepair also makes a considerable improvement on QuixBugs (31 for Java and 21 for Python at most).

==> sections/comments.tex <==

\section{Review}

\subsection{The motivation for using CoT is not clear.}

\begin{itemize}[leftmargin=*]

\item \textbf{Could you explain the principle driving the design of ThinkRepair, instead of taking fault localization as an immediate application of LLM?}

\item \textbf{While using CoT to obtain samples (fixed methods) is interesting, it’s not clear whether it is necessary. What if one uses a non-CoT prompt to get fixed examples?}

\item \textbf{Needs stronger motivation and evaluation to show the necessity of using CoT for data collection.} \em{The paper does not convince me that CoT-based fixing data collection (though interesting) is necessary and effective. I’m interested in seeing if a simpler approach (which for example directly uses existing bug-fixing data) can be as effective.}


\vspace{-0.2cm}
\end{itemize}

\subsection{The approach design incurs an overfitting issue in the evaluation.}

\begin{itemize}[leftmargin=*]


\item \textbf{Please also make clear in the paper that the bugs used for the collection phase have no overlap with those used for fixing.}

\item \textbf{Overall I think with so much information provded to ChatGPT and the fact that it probably the underlying model is familiar with QuixBugs and Defects4J (especially since it's trained in the CoT stage with it) I question the soundness of the reported results.}

\item \textbf{I question the soundness of the empirical study given that differences between the two Defects4J versions are not big, still the same projects and bugs occur in both.}

\vspace{-0.2cm}
\end{itemize}

% \subsection{Why doesn’t Table 3 include the result comparing ThinkRepair with other LLM-based techniques (e.g., ChatRepair) for method-level fault localization?}

==> sections/threats.tex <==
% \vspace{-0.2cm}
\section{Threats to Validity}

\noindent
\textbf{Internal Validity.}
The first internal threat arises from the manual validation employed to determine the correctness of the plausible patches.
To mitigate this concern, we conduct a thorough examination and comprehensive discussion of each patch, following prior work~\cite{jiang2021cure, xia2023automated, xia2022less, ye2022selfapr, ye2022neural, zhu2021syntax}.
The second one comes from potential data leakage since referenced developer patches may be part of the training data of ChatGPT.
Given that ChatGPT is a close-source model and can be accessed through API, the precise training data remains inaccessible to us. 
To tackle this issue, we follow the work~\cite{xia2022less} and initially calculate the number of correct patches generated by \toolname, which matches the reference developer patch in Defects4J V1.2.
We find that out of 98 correct patches, 24 of them aligned with the reference developer fix (24.5\%). 
Moreover, even after excluding all the correct patches (24) that aligned with the reference developer patch, \toolname is still capable of generating the correct patch for 29 unique bugs, none of which could be fixed by any previous methods.
Additionally, compared to the basic ChatGPT (i.e., BaseChatGPT), \toolname demonstrates a significant enhancement in performance (46 more correct fixes).
This demonstrates that the improved results achieved by \toolname are not merely a result of memorizing the training data.
However, to fully address this threat, it would be infeasible for an academic project since we need to retrain ChatGPT from the scratch model.

\noindent
\textbf{External Validity.}
%The main external threat to validity comes from our evaluation datasets used. 
The effectiveness observed in \toolname's performance may not be applicable across different repair datasets. 
We conduct evaluations not only on the widely-used Defects4J dataset but also on QuixBugs dataset. 
This broader evaluation scope aims to showcase the generalizability of our approach.

\begin{figure}
\vspace{-0.3cm}
    \centering
    \includegraphics[width=.65\linewidth]{figs/interaction_number.pdf}
    \caption{RQ3: The varying performance of \toolname with different interaction number}
    \label{fig:interaction}
    \vspace{-0.5cm}
\end{figure}


